FedAR: Activity and Resource-Aware Federated Learning Model for Distributed Mobile Robots

Smartphones, autonomous vehicles, and the Internet-of-things (IoT) devices are considered the primary data source for a distributed network. Due to a revolutionary breakthrough in internet availability and continuous improvement of the IoT devices capabilities, it is desirable to store data locally and perform computation at the edge, as opposed to share all local information with a centralized computation agent. A recently proposed Machine Learning (ML) algorithm called Federated Learning (FL) paves the path towards preserving data privacy, performing distributed learning, and reducing communication overhead in large-scale machine learning (ML) problems. This paper proposes an FL model by monitoring client activities and leveraging available local computing resources, particularly for resource-constrained IoT devices (e.g., mobile robots), to accelerate the learning process. We assign a trust score to each FL client, which is updated based on the client's activities. We consider a distributed mobile robot as an FL client with resource limitations either in memory, bandwidth, processor, or battery life. We consider such mobile robots as FL clients to understand their resource-constrained behavior in a real-world setting. We consider an FL client to be untrustworthy if the client infuses incorrect models or repeatedly gives slow responses during the FL process. After disregarding the ineffective and unreliable client, we perform local training on the selected FL clients. To further reduce the straggler issue, we enable an asynchronous FL mechanism by performing aggregation on the FL server without waiting for a long period to receive a particular client's response.

==> whitepaper.tex <==
Ahmed's thoughts and Ideas on the title and potential application??

Title: Agent-based Modeling to Exploit Personal and Premises Federated Surveillance Video Data

The Department of Homeland Security (DHS) obtains and retrieves a high amount of video data from various surveillance systems (e.g., CCTV cameras, vehicle-mounted cameras), and videos captured by citizens on their phones or home surveillance systems. A video of an incident can be captured by multiple cameras of a home surveillance system. Each camera may have a partial scene of an event that other cameras do not observe. In such a case, reconstruction of the overall incident and discovering valuable insight from a vast stream of video data is a challenge in terms of computation and memory usage. Besides, due to privacy, many citizens do not prefer to share their personal or premises data with a third party or an external entity. Instead of that, if we perform decision-making computation at the edge, i.e., each distributed agent autonomously identifies a potentially risky situation and notify that to the homeland security, we can significantly reduce both computational cost and time. 
Our goal of this project is to design agent-based modeling by applying Federated Learning (FL) technique on distributed agents residing within the citizens' personal and premises. In our proposed approach, an agent of a home surveillance system locally stores all captured videos from cameras, carry-out on-device model training, and performs prediction by analyzing the captured data. However, we can not achieve a satisfactory prediction accuracy if the agent's model only trained with its local data. Therefore, we propose a distributed machine learning-based Federated Learning (FL) strategy to ascertain any violation within a personal or premises. The major advantage of FL is that an agent can recognize an unseen and risky situation by learning from another home surveillance system's agent observation. Moreover, if an agent has partial information of an event and another agent has the rest of the portion, they can reconstruct the whole event through the FL procedure. It is to be noted that none of the agents needs to share their raw data with other agents or even with the server. Instead of that, every agent shares their model parameters with the server, and further, the server broadcasts the aggregated model parameters to all the available agents. That means each agent improves its model by learning from its local data and updates its model parameters using the aggregated global model information. However, any agent can pass improper model information (e.g., poisoning attack) to the server to obstruct a model training and be out of resources. To handle such inappropriate behavior and resource-outage of an agent, we propose activity and resource-aware FL schemes that can avoid bad data infusion by a home surveillance system agent and further exclude that agent from participating in the learning phase.








*******************
White paper

Sample project topics: https://cina.gmu.edu/projects/

sample related project :
https://cina.gmu.edu/projects/an-extensible-criminal-predictive-analytic-platform-cpap-for-opioid-abuse-detection-and-prediction/

https://cina.gmu.edu/projects/geospatial-technology-and-agent-based-modeling/


Title
\textbf{Distributed Machine Learning for Edge Computing in Distributed Sensor Networks 
}
The main idea is leveraging FL for handwriting recognition as well as the algorithms in new ICMLA paper.



Limit: (5) pages in length, single-spaced, 11- or 12-point font with 1" margins. 

1.	Executive Summary  \\
2.	Problem: Description of the essential problem area. \\
3.	Prior and Related Work: Discussion of prior work, related work, and state of the art. [from ACM Computing SUrvey with many related references; less than 1.5 pages \\
4.	Approach: A sufficiently detailed description of the proposed approach to address the identified problem. [here add algorithms 1 and 2 of the ICMLA paper as well as some details of your qualifying exam paper]\\
5.	Team Experience and Resources: Provide evidence supporting the team's ability to perform the proposed effort. [explain your published work in CSCI and best paper award, as well as robotics project with undergrad] \\
6.	DHS Relevance: Identify the DHS component or components most likely to be interested in the conduct and outcomes of the proposed research. [identify \\
7.	Timeline: A high level timeline for the project.\\
8.	Cost Estimate: Rough order of magnitude cost estimate for the project. \\
9.	References: Not included in page count\\


